CIBench: Evaluating Your LLMs with a Code Interpreter Plugin

While LLM-Based agents, which use external tools to solve complex problems, have made significant progress, benchmarking their ability is challenging, thereby hindering a clear understanding of their limitations. In this paper, we propose an interactive evaluation framework, named CIBench, to comprehensively assess LLMs' ability to utilize code interpreters for data science tasks. Our evaluation framework includes an evaluation dataset and two evaluation modes. The evaluation dataset is constructed using an LLM-human cooperative approach and simulates an authentic workflow by leveraging consecutive and interactive IPython sessions. The two evaluation modes assess LLMs' ability with and without human assistance. We conduct extensive experiments to analyze the ability of 24 LLMs on CIBench and provide valuable insights for future LLMs in code interpreter utilization.

==> sections/datacard.tex <==
\section{Datasheet}

\section*{1. Motivation}
\begin{enumerate}[label=\alph*)]
    \item \textbf{What was the dataset created for?}

    The dataset is created to evaluate the LLMs ability to utilize code interpreters.
    
    \item \textbf{Who created the dataset and on behalf of which entity?}

    This dataset was created by Songyang Zhang, Chuyu Zhang, Yingfan Hu, Kuikun Liu, Zerun Ma, Fengzhe Zhou, Wenwei Zhang, Xuming He, Dahua Lin, Kai Chen.
    Songyang Zhang, Yingfan Hu, Kuikun Liu, Zerun Ma, Fengzhe Zhou, Wenwei Zhang, Dahua Lin, Kai Chen are with ShanghaiAI lab. Chuyu Zhang and Xuming He are with ShanghaiTech University.
    
    \item \textbf{Who funded the creation of the dataset?}
    
    The creation of this dataset was funded by ShanghaiAI lab.
    
    \item \textbf{Any other Comments?}

    None.
\end{enumerate}

\section*{2. Composition}
\begin{enumerate}[label=\alph*)]
    \item \textbf{What do the instances that comprise the dataset represent?}
    
    Each instance is an ipynb file, containing multiple data science-related questions, such as data processing, model building, etc.
    
    \item \textbf{How many instances are there in total?}

    234 instances.
    
    \item \textbf{Does the dataset contain all possible instances or is it a sample of instances from a larger set?}

    No, this is a brand-new dataset.
    
    \item \textbf{What data does each instance consist of?}
    
    Each instance contains multiple data science-related questions. See Appendix C for an example.
    
    \item \textbf{Is there a label or target associated with each instance?}
    Yes. We provide the ground-truth code for each question.
    
    \item \textbf{Is any information missing from individual instances?}
    
    No.
    
    \item \textbf{Are relationships between individual instances made explicit?}

    There is no relation between instances.
    
    \item \textbf{Are there recommended data splits?}

    Yes. The dataset is only used for evaluation.
    
    \item \textbf{Are there any errors, sources of noise, or redundancies in the dataset?}
    
    There are almost certainly some errors in video annotations. We have done our best to minimize these.
    
    \item \textbf{Is the dataset self-contained, or does it link to or otherwise rely on external resources? (e.g., websites, tweets, other datasets)?}

    The dataset has to download additional files, like MNIST dataset.
    
    \item \textbf{Does the dataset contain data that might be considered confidential? (e.g., data that is protected by legal privilege or by doctor-patient confidentiality, data that includes the content of individuals’ non-public communications)?}

    No.
    
    \item \textbf{Does the dataset contain data that, if viewed directly, might be offensive, insulting, threatening, or might otherwise cause anxiety?}

    No.
    
    \item \textbf{Does the dataset relate to people?}

    No.
    
    \item \textbf{Does the dataset identify any subpopulations (e.g., by age, gender)?}

    No.
    
    \item \textbf{Is it possible to identify individuals (i.e., one or more natural persons), either directly or indirectly (i.e., in combination with other data) from the dataset?}

    No.
    
    \item \textbf{Does the dataset contain data that might be considered sensitive in any way (e.g., data that reveals racial or ethnic origins, sexual orientations, religious beliefs, political opinions or union memberships, or locations; financial or health data; biometric or genetic data; forms of government identification, such as social security numbers; criminal history)?}

    No.
    
    \item \textbf{Any other comments?}

    None.
\end{enumerate}

\section*{3. Collection Process}
\begin{enumerate}[label=\alph*)]
    \item \textbf{How was the data associated with each instance acquired?}

    See main paper for details.
    \item \textbf{What mechanisms or procedures were used to collect the data (e.g., hardware apparatus or sensor, manual human curation, software program, software API)?}

    We utilize LLM model and humans to generate data.
    
    \item \textbf{If the dataset is a sample from a larger set, what was the sampling strategy (e.g. deterministic, probabilistic with specific sampling probabilities)?}

    No.
    
    \item \textbf{Who was involved in the data collection process (e.g., students, crowdworkers, contractors) and how were they compensated (e.g., how much were crowdworkers paid)?}

    The authors are involved in the data collection process and are paid a fair wage.
    
    
    \item \textbf{Over what timeframe was the data collected?}

    The dataset is collected in 2023-2024.
    
    \item \textbf{Were any ethical review processes conducted (e.g., by an institutional review board)?}

    Not applicable.
    
    \item \textbf{Does the dataset relate to people?}

    No.
    
    \item \textbf{Did you collect the data from the individuals in question directly, or obtain it via third parties or other sources?}

    Not applicable.
    
    \item \textbf{Were the individuals in question notified about the data collection?}

    Not applicable.
    
    \item \textbf{Did the individuals in question consent to the collection and use of their data?}

    Not applicable.
    
    \item \textbf{If consent was obtained, were the consenting individuals provided with a mechanism to revoke their consent in the future or for certain uses?}

    Not applicable.
    
    \item \textbf{Has an analysis of the potential impact of the dataset and its use on data subjects been conducted?}

    Not applicable.
    
    \item \textbf{Any other comments?}

    None.
    
\end{enumerate}

\section*{4. Preprocessing, Cleaning and Labeling}
\begin{enumerate}[label=\alph*)]
    \item \textbf{Was any preprocessing/cleaning/labeling of the data done (e.g., discretization or bucketing, tokenization, part-of-speech tagging, SIFT feature extraction, removal of instances, processing of missing values)?}
    
    No. There is no preprocessing.
    
    \item \textbf{Was the "raw" data saved in addition to the preprocessed/cleaned/labeled data?}

    Our dataset is raw data.
    
    \item \textbf{Is the software used to preprocess/clean/label the instances available?}

    Not applicable.
    
    \item \textbf{Any other comments?}

    None.
    
\end{enumerate}

\section*{5. Uses}
\begin{enumerate}[label=\alph*)]
    \item \textbf{Has the dataset been used for any tasks already?}

    No. 
    
    \item \textbf{Is there a repository that links to any or all papers or systems that use the dataset?}

    Not applicable.
    
    \item \textbf{What (other) tasks could the dataset be used for?}

    It also can be used to evaluate the LLM's reasoning ability.
    
    \item \textbf{Is there anything about the composition of the dataset or the way it was collected and preprocessed/cleaned/labeled that might impact future uses?}

    None.
    
    \item \textbf{Are there tasks for which the dataset should not be used?}

    No.
    
    \item Any other comments?

    None.
    
\end{enumerate}

\section*{6. Distribution}
\begin{enumerate}[label=\alph*)]
    \item \textbf{Will the dataset be distributed to third parties outside of the entity on behalf of which the dataset was created?}

    Yes, the dataset will be made publicly available.
    
    \item \textbf{How will the dataset be distributed? (e.g., tarball on website, API, GitHub)?}
    
    \href{https://github.com/open-compass/opencompass/releases/download/0.2.4.rc1/cibench_dataset.zip}{github}

    \item \textbf{When will the dataset be distributed?}
    
    It will be released on \href{https://github.com/open-compass/opencompass/releases/download/0.2.4.rc1/cibench_dataset.zip}{github} soon.
    
    \item \textbf{Will the dataset be distributed under a copyright or other intellectual property (IP) license, and/or under applicable terms of use (ToU)?}

    We release our benchmark under CC BY-NC license.
    
    \item \textbf{Have any third parties imposed IP-based or other restrictions on the data associated with the instances?}

    No.
    
    \item \textbf{Do any export controls or other regulatory restrictions apply to the dataset or to individual instances?}

    No.
    
    \item \textbf{Any other comments?}

    None.
    
\end{enumerate}

\section*{7. Maintenance}
\begin{enumerate}[label=\alph*)]
    \item \textbf{Who is supporting/hosting/maintaining the dataset?}

    Chuyu Zhang
    \item\textbf{How can the owner/curator/manager of the dataset be contacted (e.g., email address)?}

    zhangchuyu@pjlab.org.cn
    
    \item \textbf{Is there an erratum?}

    Currently, there are no errors. We will update the dataset if we find errors. 
    
    \item \textbf{Will the dataset be updated (e.g., to correct labeling errors, add new instances, delete instances’)?}

    Yes.
    
    \item \textbf{If the dataset relates to people, are there applicable limits on the retention of the data associated with the instances (e.g., were individuals in question told that their
data would be retained for a fixed period of time and then deleted)?}

    Not applicable.
    
    \item \textbf{Will older versions of the dataset continue to be supported/hosted/maintained?}

    Yes, older versions of the benchmark will be maintained on our website.
    
    \item \textbf{If others want to extend/augment/build on/contribute to the dataset, is there a mechanism for them to do so?}

    Yes, make a PR on the github.
    
    \item \textbf{Any other comments?}

    None.
\end{enumerate}

==> tables/api_table.tex <==
% \begin{table*}[!t]
%     % \vspace{0.5em}
%     \caption{\textbf{API Results of \shortname.} API models result-oriented metrics are summarized here. \textbf{bold} denotes the best score among the same model scale.}
%     \label{tab:api_results}
%     \setlength{\tabcolsep}{6pt}
%     \renewcommand{\arraystretch}{1.1}
%     \centering
%     % \resizebox{\textwidth}{!}{%
%     \begin{tabular}{l|ccc|ccc|c}
%     \toprule
%     \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c|}{\textbf{\textsc{Multi Round}}} & \multicolumn{3}{c|}{\textbf{\textsc{Single Round}}} & \multirow{2}{*}{\textbf{Overall}}\\
%     % \cline{2-13}
%     % & \multicolumn{2}{c}{\textbf{\textsc{Round Overall}}}
%     \addlinespace[0.5pt]
%     & \small{num} & \small{text} & \small{vis} & \small{num} & \small{text} & \small{vis} &  \\ \midrule
%         ChatGLM\_Pro & 42.3  & 45.1  & 42.6  & 45.7  & 62.4  & 39.0  & 46.2  \\ 
%         Baichuan2\_Turbo & 39.9  & 51.7  & 38.8  & 51.5  & 70.8  & 36.4  & 48.2  \\ 
%         Claude-2 & 37.8  & 41.1  & 26.7  & 61.0  & \textbf{78.1}  & 59.7  & 50.7  \\ 
%         Qwen-Max & 55.5  & 67.8  & 50.5  & \textbf{72.2}  & 71.5  & 58.9  & 62.7  \\ 
%         GPT4-Turbo & \textbf{76.0}  & \textbf{78.9}  & \textbf{64.0}  & 70.8  & 76.5  & \textbf{67.4}  & \textbf{72.3}  \\ \bottomrule
% \end{tabular}
% % }
% \end{table*}







==> tables/icl-results.tex <==
\newcommand\redcolor[1]{\cellcolor{gray!30!red!30}{#1}}
\newcommand\bluecolor[1]{\cellcolor{gray!30!blue!30}{#1}}
\begin{table*}[ht]
\caption{
    }
    \vspace{0.5em}
    \label{tab:gpt4-main-results}
    \setlength{\tabcolsep}{4.0pt}
    \renewcommand{\arraystretch}{1.1}
    \centering
    \small
    \begin{tabular}{l|cccccccccccc|c}
    \toprule
    \multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{Instruct}} & \multicolumn{2}{c}{\textbf{Retrieve}} & \multicolumn{2}{c}{\textbf{Plan}} & \multicolumn{2}{c}{\textbf{Reason}} & \multicolumn{2}{c}{\textbf{Review}} & \multicolumn{2}{c}{\textbf{Summary}} & \multirow{2}{*}{\textbf{Average}}\\
    % \cline{2-13}
    \addlinespace[1pt]
    & \small{String} & \small{JSON} & \small{Easy} & \small{Hard} & \small{Easy} & \small{Hard} & \small{Easy} & \small{Hard} & \small{Easy} & \small{Hard} & \small{Easy} & \small{Hard} & \\ %
    \midrule
    \multicolumn{14}{l}{\redcolor{\textbf{\textit{API-based}}}} \\
    % \midrule
    ChatGPT & \\
    GPT4 & \\
    \midrule
    \multicolumn{14}{l}{\bluecolor{\textbf{\textit{Open-Sourced}}}} \\
    LLaMA2-7b   & 9.7  & 0.0  & 33.4 & 0.0  & 44.3 & 0.0  & -    & -    & -    & -    & - & - & -\\
    Vicuna-7b   & \\
    InternLM-7b & 45.2 & 11.3 & 21.9 & 0.0  & 61.9 & 5.8  & 49.8 & 2.2  & 40.3 & 0.0  & - &  - & 24.3\\
    Baichuan-7b & \\
    Qwen-7b     & 25.3 & 81.7 & 44.2 & 0.0  & 62.6 & 0.6  & 59.7 & 22.3 & 51.5 & 0.0  & - & - &  37.1\\
    ChatGLM3-6b & 69.8 & 81.2 & 53.6 & 31.7 & 54.6 & 31.8 & -    & -    & 52.3 & 38.8 & - & - &  \textbf{46.2}\\
    \midrule
    LLaMA2-13b  & 46.3 & 0.0  & 36.9 & 0.0  & 43.1 & 0.0  & 8.3  & 0.0  & 50.1 & 0.0  & - & - &  21.2\\
    Vicuna-13b  & \\
    Baichuan-14b& \\
    Qwen-14b    & 41.0 & 69.3 & 61.9 & 6.8  & 77.0 & 35.4 & 61.3 & 33.2 & 53.1 & 1.1  & - & - &  44.5\\
    WizardLM-14b& \\
    InternLM-20b& 40.8 & 57.8 & 65.1 & 0.0  & 82.2 & 13.4  & 67.3 & 32.6 & 8.7  & 34.0 & - & - & 40.5\\
    \midrule
    % Vicuna-33b & \\
    % WizardLM-33b & \\
    
    % \midrule
    LLaMA2-70b  & 69.9 & 4.0  & 56.2 & 5.9  & 61.9 & 1.1  & 41.2 & 0.0  & 49.2 & 0.9  & - & - &  30.9\\
    WizardLM-70b & \\
    \bottomrule
    \end{tabular}
    \end{table*}

==> tables/instruction_following.tex <==
\begin{table*}[ht]
    % \vspace{0.5em}
    \caption{\textbf{Action Call Rate.}}
    \label{tab:instruction_following}
    \setlength{\tabcolsep}{4pt}
    \renewcommand{\arraystretch}{1.1}
    \centering
    % \resizebox{\textwidth}{!}{%
    \begin{tabular}{l|ccc|ccc|c}
    \toprule
        \textbf{Mode} & \textbf{Multi-Round} & \textbf{Single-Round} \\
    \addlinespace[1pt]
        baichuan2-7b-chat-hf & 59.0  & 98.3  \\ 
        deepseek-7b-chat-hf & 59.5  & 84.4  \\ 
        zephyr-7b-beta-hf & 73.9  & 99.6  \\ 
        chatglm3-6b-32k-hf & 77.6  & 98.9  \\ 
        llama-2-7b-chat-hf & 79.0  & 95.2  \\ 
        yi-6b-chat-hf & 85.8  & 100.0  \\ 
        vicuna-7b-v1.5-16k-hf & 88.2  & 99.9  \\ 
        internlm-chat-7b-hf-v11 & 93.6  & 98.8  \\ 
        mistral-7b-instruct-v0.2-hf & 96.4  & 99.2  \\ 
        Ampere-7B-3.0.0-P-0.19.0 & 96.8  & 97.8  \\ 
        qwen-7b-chat-hf & 99.1  & 98.1  \\ \hline
        \textbf{Average} & 82.6  & 97.3  \\ 
\end{tabular}
% }
\end{table*}







==> tables/statistics.tex <==
\begin{figure}
\begin{minipage}[t]{.5\linewidth}
% \renewcommand\arraystretch{1.1}
\small
\captionof{table}{The statistics of the evaluation datasets in \shortname.}
\label{tab:data_stat}
\centering
    \begin{tabular}{c| c }
        \toprule
            Dataset & Test Cases \\
        \midrule
        \textsc{Instruct} & 2660\\
        \textsc{Retrieve} & 6426\\
        \textsc{Plan} & 553\\
        \textsc{Reason} & 6426\\
        \textsc{Review} & 487\\
        \textsc{Understand} & 6753\\
        \midrule
        Total & 23305\\
        \bottomrule
    \end{tabular}
\end{minipage}%
\hspace{2mm}
\begin{minipage}[t]{.45\linewidth}
    \centering
    \caption{The step count distribution of the query in \shortname.}
    \includegraphics[width=1.0\linewidth]{figures/step_cnt.png}
    \label{fig:step_dist}
\end{minipage}%

\end{figure}
